Task Attribute Distance for Few-Shot Learning: Theoretical Analysis and Applications

Few-shot learning (FSL) aims to learn novel tasks with very few labeled samples by leveraging experience from \emph{related} training tasks. In this paper, we try to understand FSL by delving into two key questions: (1) How to quantify the relationship between \emph{training} and \emph{novel} tasks? (2) How does the relationship affect the \emph{adaptation difficulty} on novel tasks for different models? To answer the two questions, we introduce Task Attribute Distance (TAD) built upon attributes as a metric to quantify the task relatedness. Unlike many existing metrics, TAD is model-agnostic, making it applicable to different FSL models. Then, we utilize TAD metric to establish a theoretical connection between task relatedness and task adaptation difficulty. By deriving the generalization error bound on a novel task, we discover how TAD measures the adaptation difficulty on novel tasks for FSL models. To validate our TAD metric and theoretical findings, we conduct experiments on three benchmarks. Our experimental results confirm that TAD metric effectively quantifies the task relatedness and reflects the adaptation difficulty on novel tasks for various FSL methods, even if some of them do not learn attributes explicitly or human-annotated attributes are not available. Finally, we present two applications of the proposed TAD metric: data augmentation and test-time intervention, which further verify its effectiveness and general applicability. The source code is available at https://github.com/hu-my/TaskAttributeDistance.

==> overleaf/sections/abandon/calculation.tex <==
\section{Model-Agnostic Task Distance Approximation}
\begin{comment}

\subsection{Distance Approximation}
In this section, we discuss practical considerations in computing the TAD on real data, where the attributes often take on discrete and finite values. 
For continuous and infinite attributes, it is possible to divide their values into many segments or discrete parts.
Therefore, we denote $V^l$ as a finite set of possible values of attribute $a^l$, and re-express the TAD in Eq \ref{eq:dis_task} as
\begin{align}
    d(\tau_i, \tau_{j}') 
    &= \frac{1}{2L\left|M\right|} \sum_{e_{kt}\in M} \sum_{l=1}^L \sum_{v\in V^l}\left| P^i_{a^l|y_k}[v]-P^j_{a^l|y_t}[v]\right|. 
    \label{eq:dis_task_v}
\end{align}
Computing the above distance is challenging as it requires finding the maximum matching $M$ with minimum weights, which is a combinatorial optimization problem.
The Hungarian algorithm \cite{kuhn1955hungarian} is commonly used to solve the matching problem, but it is computationally expensive.
%The algorithm employs a modified shortest path search in the augmenting path algorithm, and its running time is $O(V^2\log V + VE)$ or $O(V^2E)$, where $V$ is the number of vertices and $E$ is the number of edges.
Due to the high computational cost, we do not calculate this distance directly but estimate the approximation instead:
\begin{equation}
    d(\tau_i, \tau_{j}') \approx \frac{1}{2LC} \sum_{l=1}^L \sum_{v\in V^l}\left| \sum_{k=1}^C P^i_{a^l|y_k}[v]-\sum_{t=1}^C P^j_{a^l|y_t}[v]\right|, 
    \label{eq:approximation}
\end{equation}
where we assume all tasks have $C$ categories, which holds in most FSL settings.
In Eq \ref{eq:approximation}, we simplify the comparison of attribute conditional distributions between two tasks by replacing the individual differences with the average difference.
Through the above approximation, we can avoid seeking the minimum weight perfect matching %omit the problem that find a minimum-weight perfect matching 
$M$ and estimate the TAD efficiently.
    
\end{comment}

In this section, we discuss practical considerations in computing the TAD on real data, where the attributes often take on discrete and finite values. 
For continuous and infinite attributes, it is possible to divide their values into many segments or discrete parts.
Denote $V^l$ as a finite set of possible values of attribute $a^l$, we can re-express the TAD in Eq \ref{eq:dis_task} as:
\begin{align}
    d(\tau_i, \tau_{j}') 
    &= \frac{1}{2L\left|M\right|} \sum_{e_{kt}\in M} \sum_{l=1}^L \sum_{v\in V^l}\left| P^i_{a^l|y_k}[v]-P^j_{a^l|y_t}[v]\right|. 
    \label{eq:origin}
\end{align}
We denote the distance metric adopting above equation as TAD-Orig.

Computing the TAD-Orig is challenging as it requires finding the maximum matching $M$ with minimum weights, which is a combinatorial optimization problem.
The Hungarian algorithm \cite{kuhn1955hungarian} is commonly used to solve the matching problem, but it is computationally expensive.
%The algorithm employs a modified shortest path search in the augmenting path algorithm, and its running time is $O(V^2\log V + VE)$ or $O(V^2E)$, where $V$ is the number of vertices and $E$ is the number of edges.
Due to the high computational cost, we show some variants by estimating the approximation instead of calculating the TAD-Orig directly:
\begin{equation}
    d(\tau_i, \tau_{j}') = \frac{1}{2LC} \sum_{l=1}^L \sum_{v\in V^l}\left| \sum_{k=1}^C P^i_{a^l|y_k}[v]-\sum_{t=1}^C P^j_{a^l|y_t}[v]\right|, 
    \label{eq:approximation}
\end{equation}
where we assume all tasks have $C$ categories, which holds in most FSL settings.
We denote the distance metric adopting the Eq \ref{eq:approximation} as TAD-Average.
In the TAD-Average, we simplify the comparison of attribute conditional distributions between two tasks by replacing the individual differences with the average difference.
Through the above approximation, we can avoid seeking the minimum weight perfect matching $M$ and estimate the distance efficiently.
Without specific instructions, we will utilize the TAD-Average in the following experiments, as we find that TAD-Average has similar performance with TAD-Orig but calculates more efficiently.

\begin{comment}
    
\subsection{Attributes Auto-Annotation}
\label{Sec 5.2}
As stated before, our proposed theory and TAD metric rely on category-level attribute annotations that are possibly unavailable for some few-shot benchmarks, like \emph{mini}ImageNet \cite{vinyals2016matchnet}.
To address this issue, we propose a solution to auto-annotate attributes using a pretrained CLIP \cite{radford2021CLIP} model, which has demonstrated impressive zero-shot classification ability.
We first pre-define 14 attribute labels based on pattern, shape, and texture.
Then we create two descriptions for each attribute, such as ``a photo has shape of round'' and ``a photo has no shape of round'', which are used as text inputs for CLIP.
We formulate the annotation problem as 14 attribute binary classification problems for each image using CLIP model.
After that, we gather the attribute predictions of all images within the same category, which provides rough category-level attribute information while greatly reduces the cost of attribute annotations.
With the above auto-annotation process, we can obtain the category-level attributes for \emph{mini}ImageNet in just 5 minutes.

\end{comment}

==> overleaf/sections/abandon/problem_setting.tex <==
\section{Problem Setting}
In few-shot learning problem, a model observes $n$ different training tasks $\{\tau_i\}_{i=1}^n$ with each task represented as a pair $\tau_i=(\mathcal{D}_i, S_i), 1\leq i\leq n$. 
$\mathcal{D}_i$ is an unknown data distribution over the input space $\mathcal{X}$ and label space $\mathcal{Y}_i$. $S_i=\{(x_k, y_k)|(x_k,y_k)\sim \mathcal{D}_i\}_{k=1}^{m_i}$ represents an observed training set drawn from $\mathcal{D}_i$.  
With a model trained on the $n$ training tasks, our target is to adapt and evaluate it on $t$ novel test tasks $\tau_{j}'=(\mathcal{D}_{j}',S_{j}')$, $1\leq j\leq t$. 
$\mathcal{D}_{j}'$ is an unknown data distribution over $\mathcal{X}$ and $\mathcal{Y}_{j}'$, and $S_{j}'$ is a labeled dataset drawn from $\mathcal{D}_j'$.  
Note that, in few-shot learning, the labeled data for each category is very limited, and the categories in training tasks $\{\tau_i\}_{i=1}^n$ will not appear in novel tasks $\{\tau_j'\}_{j=1}^t$, which means $ \mathcal{Y}_i\cap\mathcal{Y}'_j = \emptyset$,  $\forall i\in\{1, ..., n\},j\in\{1, ..., t\}$.


==> overleaf/sections/abandon/theory.tex <==
\section{Generalization Analysis of Attribute-based Few-shot Learning}
The key to answering the two questions we raised above lies in a proper metric that quantifies task relatedness and contributes to the generalization error on a novel task. 
In this section, we begin by introducing the Task Attribute Distance (TAD), which first measures the category relationship through attribute conditional distributions, based on which the relationship between tasks is measured as well.
Then, to facilitate our theoretical analysis, we introduce a meta-learning framework with attribute learning.
Finally, we provide theoretical proof that establishes a connection between the proposed TAD metric and the generalization error bound on a novel task.

\subsection{Task Attribute Distance}
To measure the relationship between two categories $y_k$ and $y_t$, a natural idea is to measure the divergence of class-conditional distributions.
An intuitive divergence measure is the $L_1$ or total variation distance \cite{gibbs2002tv_dis}, which is defined as
\begin{align}
    d(y_k, y_t) &= d_{TV}(p(x|y_k), p(x|y_t)) \notag\\
    &= \sup_{B\in\mathcal{B}}\left| P_{x|y_k}[B]-P_{x|y_t}[B]\right|,
\end{align}
where $\mathcal{B}$ is the set of measurable subsets under distributions $p(x|y_k)$ and $p(x|y_t)$, and $P_{x|y_k}[B]$ denotes the probability of subset $B\in\mathcal{B}$ under $p(x|y_k)$. 
Unfortunately this distance is often hard to compute, because the distribution of $p(x|y)$ is usually unknown and the set $\mathcal{B}$ is often infinite.

In this paper, we introduce attributes to overcome the above limitation because the values of attributes are usually discrete and finite.
The basic idea is based on the \emph{attribute compositionality hypothesis} presented in the introduction section. 
Specifically, the distance between two categories can be measured by the difference between the corresponding attribute conditional distributions.
Follow the above idea, let $\mathcal{A}$ be the attribute space spanned by $L$ attribute variables $\{a^l\}_{l=1}^L$, we define the \emph{distance between two categories} $y_k$ and $y_t$ on $L$ attribute variables as:
\begin{align}
    d_{\mathcal{A}}(y_k, y_t) &= \frac{1}{L}\sum_{l=1}^L d_{TV}(p(a^l|y_k), p(a^l|y_t)) \\ 
     &= \frac{1}{L} \sum_{l=1}^L \sup_{B\in\mathcal{B}^l}\left| P_{a^l|y_k}[B]-P_{a^l|y_t}[B]\right|,
    \label{eq:dis_category}
\end{align}
where $\mathcal{B}^l$ is the set of measurable subsets under attribute conditional distributions $p(a^l|y_k)$ and $p(a^l|y_t)$, and $\mathcal{B}^l$ is a finite set if the values of variable $a^l$ are finite.

Based on the distance between categories, we then define the distance metric between training and novel test tasks.
To this end, we represent the set of categories in training task $\tau_i$ and the set of categories in novel task $\tau_{j}'$ as two disjoint vertex sets respectively, and construct a weighted bipartite graph $G$ between the two vertex sets, where each node denotes a category and each edge weight represents the distance between two categories in $\tau_i, \tau_{j}'$ respectively.
Let $M=\{e_{kt}\}$ denote a maximum matching of  $G$, which contains the largest possible number of edges and any two edges do not connect the same vertex.
We choose $M$ with minimum weights and define the \emph{task distance} as
\begin{align}
    d(\tau_i, \tau_{j}') &= \frac{1}{\left|M\right|} \sum_{e_{kt}\in M} d_{\mathcal{A}}(y_k, y_t) \\
    &=  \frac{1}{L\left|M\right|} \sum_{e_{kt}\in M} \sum_{l=1}^L d_{TV}(p(a^l|y_k), p(a^l|y_t)),
    \label{eq:dis_task}
\end{align}
where $\left|M\right|$ is the number of edges in matching $M$.
From this definition, if the two tasks $\tau_i, \tau_{j}'$ are identical, the task distance $d(\tau_i, \tau_{j}')$ is equal to 0.
We call the task distance $d(\tau_i, \tau_{j}')$ as the Task Attribute Distance (TAD).
Additionally, the TAD is invariant to the permutation of categories in tasks.
In other words, modifying the numeric order of categories in $\tau_i$ or $\tau_{j}'$ does not affect their distance $d(\tau_i, \tau_{j}')$.
To emphasize the attribute conditional distributions with respect to different tasks, we hereinafter add task indexes on the distribution and probability notations, like $p^i(a^l|y_k)$ and $P^i_{a^l|y_k}[B]$, although the true distributions are task agnostic.

\subsection{A Specific Few-Shot Learning Framework}
\label{Sec 4.2.1}
To facilitate the subsequent theoretical analysis, we consider a meta-learning framework with attribute learning.
In this framework, a meta-learner $f_\theta: \mathcal{X}\rightarrow \mathcal{A}$ parameterized by $\theta$ learns the mapping from a sample $x\in\mathcal{X}$ to attributes $a\in\mathcal{A}$, and a task-specific base-learner $g_{\phi_i}: \mathcal{A}\rightarrow \mathcal{Y}_i$ parameterized by $\phi_i$ learns the mapping from attributes $a\in\mathcal{A}$ to a class label $y\in\mathcal{Y}_i$ for training task $\tau_i$.
During training, $f_\theta$ is meta-learned from $n$ different training tasks.
To adapt to a novel task $\tau_{j}'$, we fix $f_\theta$ and train a new base-learner $g_{\phi_{j}'}$ parameterized by $\phi_{j}'$ using few labeled samples $S_j'$. 

In the following theoretical deduction, we will denote $p_\theta(a,y)\triangleq p(f_{\theta}(x),y)$ as a joint distribution over $\mathcal{A}\times\mathcal{Y}$ induced by the meta-learned mapping $f_\theta$. 
Further, with the induced conditional distribution $p_\theta(a|y)$, we can compute the distance between task $\tau_i$ and $\tau_j'$ as 
\begin{align}
    d_\theta(\tau_i, \tau_{j}') &= \frac{1}{L\left|M\right|}\sum_{e_{kt}\in M} \sum_{l=1}^L d_{TV}(p_\theta^i(a^l|y_k), p_\theta^j(a^l|y_t)).
\end{align}
Note that $d(\tau_i, \tau_j')$ (as defined in Eq.\ref{eq:dis_task}) computed based on $p(a|y)$ is the model-agnostic distance metric, while $d_\theta(\tau_i, \tau_j')$ is a model-related one since it relies on the meta-learned mapping $f_\theta$.

\subsection{Theoretical Analysis on Generalization}
As for the above meta-learning framework, we provide theoretical analysis of the generalization error on a novel task, in terms of the proposed TAD metric.
We define the generalization error and empirical error of the meta-learner $f_\theta$ on novel task $\tau_{j}'$ as
\begin{align*}
    \epsilon(f_\theta, \tau_{j}')&=\mathbb{E}_{(x,y)\sim \mathcal{D}_{j}'}[\mathbb{I}(g_{\phi_{j}'}(f_\theta(x))\neq y)], \\
    \hat{\epsilon}(f_\theta, \tau_{j}')&=\frac{1}{m_{j}'} \sum_{k=1}^{m_{j}'}\mathbb{I}(g_{\phi_{j}'}(f_\theta(x_k))\neq y_k), \notag
\end{align*}
where $\phi_{j}'$ is the parameters of $g_\phi$ learned from labeled samples $S_{j}'$ given $f_\theta$, and ${m_j'}=\left|S_{j}'\right|$ is the number of labeled samples in $S_{j}'$.
$\mathbb{I}$ denotes the indicator function.
Similarly, we can define the generalization error $\epsilon(f_\theta, \tau_i)$ and empirical error $\hat{\epsilon}(f_\theta, \tau_i)$ for training task $\tau_i$.
With these definitions, we will proceed by introducing an auxiliary lemma, and then stating our main theoretical results.
All detailed proofs of the following lemma and theorems are in the Appendix. 

\begin{lemma}
    Let $\mathcal{A}$ be the attribute space, $L$ be the number of attributes.
    %For the conditional distribution $p(a|y)$, 
    Assume all attributes are independent of each other given the class label, i.e. $p(a|y) = \prod_{l=1}^Lp(a^l|y)$.
    For all $a_i \in \mathcal{A}$ and any two categories $y_k, y_t$, the following inequality holds:
    \begin{equation}
        \sum_{a_i\in\mathcal{A}}\left|p(a_i|y_k)-p(a_i|y_t)\right| \leq d_{\mathcal{A}}(y_k, y_t) +  \Delta,
        \label{eq:distance ineq}
    \end{equation}
    where $d_{\mathcal{A}}(y_k, y_t)$ is the distance as defined in Eq.\ref{eq:dis_category} and $\Delta=\sum_{a_i\in\mathcal{A}}\frac{1}{2L}\sum_{l=1}^L(p(a^l_i|y_k)+p(a^l_i|y_t))$.
    \label{lemma 1}
\end{lemma}
Lemma \ref{lemma 1} says that under the attribute conditional independence assumption, the distance between two attribute conditional distributions $p(a|y_k), p(a|y_t)$ over attribute space $\mathcal{A}$ is %be spanned by 
bounded by the defined distance $d(y_k, y_t)$ and a non-negative term $\Delta$.
This result enables us to make use of the defined TAD metric in deriving the generalization error bound, leading to the following theoretical results.

\begin{theorem}
    With the same notation and assumptions as in Lemma \ref{lemma 1}, %let $\mathcal{H}$ be the hypothesis space of the meta-learning method (introduced in Sec. 4.2) with VC-dimension $d$, 
    let $\mathcal{H}$ be the hypothesis space with VC-dimension $d$, 
    $f_\theta$ and $g_\phi$ be the meta-learner and the base-learner as introduced in Sec \ref{Sec 4.2.1} respectively. 
    Denote $g_{\phi^*}$ as the best base-learner on some specific tasks given a fixed meta-learner $f_\theta$.
    For any single training task $\tau_i=(\mathcal{D}_i, S_i)$ and a novel task $\tau_{j}'=(\mathcal{D}_{j}', S_{j}')$, suppose the number of categories in the two tasks is the same, then with probability at least $1-\delta$, $\forall g_\phi\circ f_\theta\in\mathcal{H}$, we have 
    \begin{align}
         \epsilon(f_\theta, \tau_{j}')&\leq 
            \hat{\epsilon}(f_\theta, \tau_i) + \sqrt{\frac{4}{m_i}(d\log\frac{2em_i}{d}+\log\frac{4}{\delta})}
            \notag \\ &+ d_\theta(\tau_i, \tau_{j}') + \Delta' + \lambda, 
            \label{theorem 1}
    \end{align}
    where $\lambda=\lambda_i+\lambda_j'$ is the generalization error of $g_{\phi^*}$ and $f_\theta$ on the two tasks, i.e., 
    % and $\lambda_i, \lambda_t$ are the generalization error of the best base-learner $g_{\phi^*}$ with a fixed $f_\theta$ on task $\tau_i, \tau_t'$ respectively.
    $\lambda_i=\mathbb{E}_{(x,y)\sim \mathcal{D}_i}[\mathbb{I}(g_{\phi_{i}^*}(f_\theta(x))\neq y)]$, $\lambda_j'=\mathbb{E}_{(x,y)\sim \mathcal{D}_{j}'}[\mathbb{I}(g_{\phi_{j}'^*}(f_\theta(x))\neq y)]$. $\Delta'$ is a term depending on learned base-learners $g_{\phi_i}, g_{\phi_j'}$ and the best base-learners $g_{\phi_i^*}, g_{\phi_j'^*}$.
    \label{theorem 1}
\end{theorem}

Theoretically, the generalization error on a novel task is bounded by the the training task empirical error $\hat{\epsilon}(f_\theta, \tau_i)$ plus four terms: 
the second term $d_\theta(\tau_i, \tau_{j}')$ is the model-related distance between $\tau_i$ and $\tau_{j}'$, which is derived based on Lemma \ref{lemma 1};
the third term $\Delta'$ reflects the classification ability of $g_\phi$, which converges to zero if the learned base-learners are equal to the best ones for both tasks;
the last term $\lambda$ is the generalization error of $f_\theta$ and $g_{\phi^*}$, which depends on the attribute discrimination ability of $f_\theta$ and the hypothesis space of base-learner $g_\phi$.
% For a complex neural networks, if $f_\theta$ has a good attribute discrimination ability, this term usually converges to zero.
For a reasonable hypothesis space, if $f_\theta$ has a good attribute discrimination ability on both tasks, the last term usually converges to zero. 
Next we generalize this bound to the setting of $n$ training tasks.

\begin{corollary}
   With the same notation and assumptions as Theorem 1, 
    for $n$ training tasks $\{\tau_i\}_{i=1}^n$ and a novel task $\tau_{j}'$, 
    define $\hat{\epsilon}(f_\theta, \tau_{i=1}^n)=\frac{1}{n}\sum_{i=1}^n \hat{\epsilon}(f_\theta, \tau_i)$, then with probability at least $1-\delta$, $\forall g_\phi\circ f_\theta\in\mathcal{H}$, we have
    \begin{align}
        \epsilon(f_\theta, \tau_{j}')&\leq 
            \hat{\epsilon}(f_\theta, \tau_{i=1}^n) + \frac{1}{n}\sum_{i=1}^n\sqrt{\frac{4}{m_i}(d\log\frac{2em_i}{d}+\log\frac{4}{\delta})}
            \notag \\ 
            & + \frac{1}{n}\sum_{i=1}^n d_\theta(\tau_i, \tau_{j}') + \Delta' + \lambda, 
            \label{eq:corollary 1}
    \end{align}
    where $\lambda=\frac{1}{n}\sum_{i=1}^n \lambda_i + \lambda_j'$, and $\Delta'$ is a term depending on the learned base-learners $\{g_{\phi_i}\}_{i=1}^n, g_{\phi_j'
    }$ and the best base-learners $\{g_{\phi_i^*}\}_{i=1}^n, g_{\phi_j'^*}$.
    \label{corollary 1}
\end{corollary}
Corollary \ref{corollary 1} is a straightforward extension of Theorem \ref{theorem 1}, in which we consider multiple training tasks instead of a single training task.
In Corollary \ref{corollary 1}, the generalization error on a novel task $\tau_{j}'$ is  bounded partially by the average distance between task $\tau_{j}'$ and $n$  training tasks.
Note that the distance $d_\theta(\tau_i, \tau_j')$ used in the bound is %in the bound is defined on the mapping $f_\theta$, which maps each sample point $x\in\mathcal{X}$ to $a\in\mathcal{A}$, thus is a 
model-related.
Next, we further derive the relationship between model-related distance and model-agnostic distance as follows.

\begin{definition}[\textcolor{black}{$\epsilon$-approximation Network}]
    \label{definition 1}
    A learner $h$ is called an $\epsilon$-approximation network for a task $\tau$ if it is trained using the training set $S$ such that the generalization error is less than $\epsilon$, for a given $0\leq\epsilon\leq 1$.
\end{definition}

\begin{theorem}
   \label{theorem 2}
    With the same notation and assumptions as in Corollary \ref{corollary 1}, assume that the conditional distribution $p(x|a^l)$ is task agnostic, 
    \textcolor{black}{and the meta-learner $f_{\theta}$ is an $\epsilon$-approximation network for $n$ training tasks.
    If $\epsilon$ tends to zeros, the following equality holds:}
    \begin{align}
            \frac{1}{n}\sum_{i=1}^nd_\theta(\tau_i, \tau_{j}')&\leq\frac{1}{n}\sum_{i=1}^nd(\tau_i, \tau_{j}').
    \end{align}
\end{theorem}

Theorem \ref{theorem 2} shows that when  the meta-learner $f_{\theta}$ is in the proximity of the true labeling function $f:\mathcal{X}\rightarrow\mathcal{A}$ for $n$ training tasks, the model-related average distance $\frac{1}{n}\sum_{i=1}^nd_\theta(\tau_i, \tau_{j}')$ can be bounded by the average TAD $\frac{1}{n}\sum_{i=1}^nd(\tau_i, \tau_{j}')$.
Based on the universal approximation theorem  \cite{hornik1989universe, farago1993strong} and the same assumption as in Theorem \ref{theorem 2}, if $g_\phi\circ f_\theta$ is a complex enough neural network, the second and fourth terms on the r.h.s. of Eq.~(\ref{eq:corollary 1}) in Corollary \ref{corollary 1} will converge to $0$, the first term $\hat{\epsilon}(f_\theta, \tau_{i=1}^n)$ and $\frac{1}{n}\sum_{i=1}^n \lambda_i$ in the last term will converge to Bayes risk \cite{dougherty2012prc}.
We assume the Bayes risk is small enough, so that it can be ignored.
In this case, the generalization error on novel task $\tau_j'$ is only bounded by $\lambda_j'$ and the average TAD, i.e. $\epsilon(f_\theta,\tau_j')\leq \lambda_j'+\frac{1}{n}\sum_{i=1}^nd(\tau_i, \tau_j')$.
Note that the average TAD is independent of models, thus we can rely solely on the TAD metric to measure the adaptation difficulty of each novel task, without the need for training any models.

\textcolor{black}{We note that numerous widely-used FSL methods, like metric-based or transfer-based models, can be consider a special form of the attribute-based meta-learning framework, as they map input image to unnormalized densities.
Under this interpretation, the TAD metric can be a general measure to quantify task relatedness and adaptation difficulty for various FSL model.
we try to demonstrate this point in experiments.}


==> overleaf/sections/experiments.tex <==
\section{Experiments}
In this section, we conduct experiments to validate our theoretical results and explore the generality of the proposed TAD metric in quantifying task relatedness and measuring task adaptation difficulty. 
Firstly, we evaluate our TAD metric in a scenario where human-annotated attributes are available and the training/novel tasks are sampled from the same dataset but with different categories. 
Next, we test the TAD in a more general and challenging scenario where human-annotated attributes are not available and the training tasks are constructed by sampling categories from  different datasets.

\subsection{Setups}
\textbf{Datasets:} 
We choose three widely used benchmarks:
(1) CUB-200-2011 (\textbf{CUB}) \cite{wah2011CUB}: CUB is a fine-grained dataset of birds, which has 200 bird classes and 11,788 images in total.
We follow \cite{kang2021renet} to split the dataset into 100 training classes, 50 validation classes and 50 test classes.
As a fine-grained dataset, CUB provides part-based annotations, such as beak, wing and tail of a bird.
Each part is annotated by a bounding box and some attribute labels.
%For example, bill part has attributes of bill shape, bill color and bill length.
%In CUB, a total number of 15 parts, 28 attribute groups, and 312 attribute labels are available.
Because the provided attribute labels are noisy, we denoise them by majority voting, as in \cite{koh2020conceptbottleneck}.
After the pre-processing, we acquire 109 binary category-level attribute labels.
(2) SUN with Attribute (\textbf{SUN}) \cite{patterson2014sun}: 
SUN is a scene classification dataset, which contains 14,340 images for 717 scene classes with 102 scene attributes.
In following experiments, We split the dataset into 430/215/72 classes for training/validation/test, respectively.
(3) \textbf{\emph{mini}ImageNet} \cite{vinyals2016matchnet}: \emph{mini}ImageNet is a subset of ImageNet consisting of 60,000 images uniformly distributed over 100 object classes. 
% The train/validation/test splits consist of 64/16/20 object classes, respectively.
Note that, different with CUB and SUN, \emph{mini}ImageNet does not provide the attribute annotations, which means category-level attribute annotations are not available.
Following \cite{chen2019baseline++}, we consider the \emph{cross-dataset scenario} from \emph{mini}ImageNet to CUB, where we use 100 classes of \emph{mini}ImageNet as training classes, and the 50 validation and 50 test classes from CUB.

\input{overleaf/sections/tab_fig/human-ann_apnet.tex}

\textbf{Attribute Prototypical Network:} 
Our theoretical analysis is based on a specific meta-learning framework with attribute learning (proposed in Sec \ref{Sec 4.2.1}).
Thus, we first instantiate a simple model under that framework as an example to verify our theory.
%We instantiate a simple model, following the modified meta-learning framework in \cref{Sec 4.2.1}, to verify the proposed theory. 
Specifically, we adopt a four-layer convolution network (Conv-4) with an additional MLP as the meta-learner $f_\theta$. 
The convolutional network extracts feature representations from images, then the MLP takes features as input and predicts attribute labels. 
For base-learner $g_{\phi_i}$ parameterized by $\phi_i$, we simply choose an non-parametric base-learner like ProtoNet \cite{snell2017prototypical},
which takes the attributes outputted by $f_\theta$ as input to calculate cosine distance between test samples and attribute prototypes, then predicts the target label.
We call this method as \emph{Attribute Prototypical Network} (APNet).
We train APNet by simultaneously minimizing the attribute classification loss and the few-shot classification loss.
See more details of APNet in the Appendix B.

\textbf{Other FSL Methods:}
Besides of APNet, we choose five classical FSL methods in the following experiments, since they cover a diverse set of approaches to few-shot learning: (1) Matching Network (MatchingNet) \cite{vinyals2016matchnet}, (2) Prototypical Network (ProtoNet) \cite{snell2017prototypical}, (3) Relation Network (RelationNet) \cite{sung2018relationnet}, (4) Model Agnostic Meta-Learning (MAML) \cite{finn2017maml} and (5) Baseline++ \cite{chen2019baseline++}.
Note that these FSL methods, unlike the above APNet, do not use attribute annotations during training.
See more implementation and experimental details in the Appendix C.

\subsection{Task Attribute Distance with Human-annotated Attributes}
\textbf{Linear relationship under limited samples:}
According to Theorem \ref{theorem 2}, if the meta-learner $f_\theta$ is in the proximity of the true labeling function $f:\mathcal{X}\rightarrow\mathcal{A}$ for $n$ training tasks, the TAD serves as a metric to measure the adaptation difficulty on a novel task.
Although this proximity condition may hold with an infinite number of labeled samples when learning parameter $\theta$, collecting such a number of samples is impractical in real-world applications,  especially for few-shot learning.
Thus, we try to empirically verify our theoretical result with limited labeled samples for each task.
We train our APNet on CUB and SUN dataset, then use the provided attribute annotations to calculate the average distance $\frac{1}{n}\sum_{i=1}^nd(\tau_i, \tau_j')$ between each novel task $\tau_{j}'$ and $n$ training tasks $\{\tau_{i}\}_{i=1}^n$, respectively. 
For simplicity, we sample $n=100,000$ training tasks to estimate the distances to $2,400$ novel tasks.
Following $N$-way $K$-shot setting, each task only contains $N*K$ labeled samples for training or fine-tuning models.
Fig. \ref{fig:distance and task accuracy} shows the task distance and the corresponding accuracy on novel tasks for APNet.
We can observe that as the distance increases, the accuracy of APNet decreases in both 5-way 1-shot and 5-way 5-shot settings on CUB and SUN.
These results verify that TAD can characterize model's generalization error on each novel task and measure the task adaptation difficulty effectively, even with limited labeled samples for training and fine-tuning models.
Interestingly, we also find a \textbf{linear relationship} between task distance and accuracy in Fig.  \ref{fig:distance and task accuracy}: as the distance increases, the accuracy of APNet decreases \textbf{linearly} in all datasets and settings.
Note that the confidence interval in Fig. \ref{fig:distance and task accuracy} is much larger for the last a few points.
We argue this is because these distance intervals contain fewer novel tasks, thus the average accuracy of novel tasks in the interval is more easily affected by random factors.

\textbf{The number of labeled samples:}
Additionally, in Fig. \ref{fig:distance and task accuracy}, when comparing 1-shot and 5-shot results with the same distance interval, we find that the increase of accuracy varies at different distance intervals.
For instance, on the CUB dataset (comparing Fig. \ref{fig:apnet-a} with Fig. \ref{fig:apnet-b}), when the task distance is 0.14, APNet shows an improvement of approximately 10\% in accuracy for the 5-shot setting over the 1-shot setting, whereas it shows an improvement of around 15\% for the distance of 0.20. 
This suggests that increasing the number of labeled samples is more effective for harder tasks.
One possible explanation is that as the task distance increases, less knowledge can be transferred from training tasks, making it harder for models to adapt to the novel task. 
Hence, more information from the novel task is required for adaptation, and the model’s performance get more benefit from extra samples.

\input{overleaf/sections/tab_fig/human-ann_others.tex}

\input{overleaf/sections/tab_fig/auto-ann_others.tex}

\textbf{Other FSL models:}
We have shown that the average TAD can effectively reflect the task adaption difficulty for APNet.
A natural question is whether the calculated task distance can be directly applied to other FSL methods, even if they do not follow the specific meta-learning framework and do not use the attributes during training.
We try to empirically explore this question. 
With the same distance estimation and experimental setting, we conduct experiments with five different FSL methods on CUB and SUN.
Fig. \ref{fig:distance and task accuracy of other methods} shows the task distance and the corresponding accuracy of 2,400 novel test tasks for them.
We observe similar results that with the increase of task distance, the accuracy of all FSL models tends to decrease linearly.
This indicates that even though these FSL methods do not use the attribute annotations during training, they 
implicitly learn mixture of attributes in their representations. 
Therefore, attribute-based distance can still reflect the task adaptation difficulty for them. 
These results demonstrate the generality of the proposed TAD metric, and provide some insight into the transferable knowledge that different FSL models have learned from training tasks. 

\subsection{Task Attribute Distance with Auto-annotated Attributes}
\textbf{Attribute Auto-Annotation:}
As stated before, our proposed theory and TAD metric rely on category-level attribute annotations that are possibly unavailable for some few-shot benchmarks, like \emph{mini}ImageNet \cite{vinyals2016matchnet}.
To address this issue, we propose a solution to auto-annotate attributes using a pretrained CLIP \cite{radford2021CLIP} model, which has demonstrated impressive zero-shot classification ability.
We follow previous work \cite{russakovsky2010attribute} and pre-define 14 attribute labels (See the details in Tab. \ref{tab:attribute list}) based on pattern, shape, and texture.
Then we create two descriptions for each attribute, such as ``a photo has shape of round'' and ``a photo has no shape of round'', which are used as text inputs for CLIP.
We formulate the annotation problem as 14 attribute binary classification problems for each image using CLIP model.
After that, we gather the attribute predictions of all images within the same category, which provides rough category-level attribute information while greatly reduces the cost of attribute annotations.
With the above auto-annotation process, we can obtain the category-level attributes for \emph{mini}ImageNet in just 5 minutes.

\input{overleaf/sections/tab_fig/predefined-attributes.tex}

\textbf{Cross-dataset generalization:}
Another interesting question is how to utilize the proposed TAD metric in situations where human-annotated attributes are either unavailable or expensive to obtain. 
One classic example is the cross-domain few-shot learning problem, since it requires the annotation of distinct datasets with a common attribute set.
To address this challenge, we use the auto-annotation method described in previous section to annotate the attributes for both \emph{mini}ImageNet and CUB. 
We then train the above FSL models on the cross-dataset scenario from \emph{mini}ImageNet to CUB, and estimate the average task distance with the auto-annotated attributes.
Fig. \ref{fig:cross-a} illustrates the distance and corresponding accuracy of 2,400 novel test tasks with the auto-annotated attributes. 
We can find that, with the increase of task distance, the accuracy of different models tends to decrease.
This phenomenon is consistent with our previous findings and shows the proposed TAD metric still works with auto-annotated attributes.
Besides, we selectively remove some attributes to explore the influence of them in the distance-accuracy curve. 
Fig. \ref{fig:cross-b}, \ref{fig:cross-c}, \ref{fig:cross-d} show that the exclusion of pattern, shape, and texture attributes exhibits varying degrees of influence on the decreasing tendency. 
Notably, we discover that texture attributes are more importance than others, as indicated by the more pronounced fluctuations in the curve.

\textbf{Cross-dataset distance:}
Next, we explore a common underlying hypothesis in many cross-domain few-shot learning (CD-FSL) works: the category gaps across dataset are usually larger than within a dataset, resulting in sampled training tasks less related to novel tasks.
Building on this hypothesis, the CD-FSL is considered as a more challenging problem.
We try to verify this hypothesis based on our TAD metric.
More specifically, we collect the distance distributions among 2,400 novel tasks under two scenarios: (1) within-dataset scenario: the training and novel tasks are sampled from the same dataset, although their categories are not overlapped; (2) cross-dataset scenario: the training and novel tasks are sampled from different datasets, and their categories are also not overlapped.
For within-dataset scenario, we split the total 100 classes of miniImageNet into 64/16/20 classes for training/validation/test, respectively.
For cross-dataset scenario, we use the same 64 classes of miniImageNet as training classes, and the 50 validation and 50 test classes from CUB.
We use the same auto-annotated attributes for TAD computation in the two scenarios.
Fig. \ref{fig:distance distribution} shows the distance distributions among 2,400 novel test tasks under the two scenarios.
We find that, the distance distributions under the two scenarios approximately follows the Gamma distributions.
However, the mean distance of cross-dataset scenario is much larger than that of within-dataset scenario.
This result demonstrates that although there are no class overlaps between training and novel tasks, tasks sampled from different dataset (e.g. miniImageNet and CUB) are less related than sampled from the same dataset (e.g. both from miniImageNet).

\input{overleaf/sections/tab_fig/auto-ann_distance_distribution.tex}

\input{overleaf/sections/tab_fig/application_partial.tex}

\textbf{Training with partial versus all tasks:}
Using the proposed TAD, we can also investigate whether training on all available training tasks leads to better generalization compared to training on only the most related ones. 
While it is generally expected that training with more tasks helps to improve generalization, it remains a question whether this holds for heterogeneous data. 
To explore this, we follow the experimental setup of the cross-dataset scenario and select these less related training tasks based on their calculated task distances. 
We collect the classes in the selected tasks, compute the frequency of each class, and remove the most frequent 36 classes (out of a total of 100 classes in \emph{mini}ImageNet). 
We then reconstruct training tasks based on the remaining 64 classes in \emph{mini}ImageNet and retrain five FSL models. The results are presented in Tab. \ref{tab:all vs part}. It can be observed that incorporating more heterogeneous data that is less related to the novel tasks may not lead to much improvement ( %only 1-2\% 
for ProtoNet, RelationNet and MAML), but could even result in performance degradation ( %2-3\% 
for MatchingNet and Baseline++). This result may inspire future research on how to better utilize heterogeneous data to improve the few-shot learning performance of models.

\begin{comment}

\paragraph{Human-annotated Attributes}
Table [] illustrates the results of different metrics on the CUB and SUN datasets. 
We find that, with human-annotated attributes, TAD-Orig and TAD-Average significantly outperforms other three methods in identifying more challenging novel tasks across all FSL models, demonstrating the effectiveness of TAD metrics. 
Furthermore, TAD-Average achieves similar performance with TAD-Orig, which showcase that approximating Eq \ref{eq:origin} with Eq \ref{eq:approximation} is effective but more efficiently.

\paragraph{Auto-annotated Attributes}
Following previous setting in Section XX, we consider a cross-dataset scenario from \emph{mini}Imagenet to CUB. 
In this scenario, human annotated attributes are unavailable, thereby a pre-trained CLIP model is used to annotate attributes for the calculation of TAD.
Table [] illustrates the results of different metrics on the cross-dataset scenario.
We can find that TAD metric can achieve comparable results with other three methods even when the human-annotated attributes are unavailable.
    
\end{comment}


\input{overleaf/sections/tab_fig/ablation_sampled_task.tex}

\subsection{\textcolor{black}{Ablation Analysis}}
In this section, we explore multiple factors of our TAD metric, and show their influences on measuring adaptation difficulty for novel tasks.

\textbf{The number of sampled training tasks.}
In previous experiments, we randomly select $n$ different training tasks from training categories.
Subsequently, we calculate the average distance between these selected tasks and a novel task with TAD metric to measure the adaptation difficulty.
As a beginning, we first investigate the impact of the number of sampled training tasks, denoted as $n$, on the measuring of task adaptation difficulty.
We explore different values for $n$ within the set $\{100, 1000, 10000, 100000\}$, and conduct experiments using APNet model on the CUB dataset.
Fig. \ref{fig:sampled tasks} shows the distance-accuracy curves corresponding to different values of $n$.
We can find that, as the task distance increases, the accuracy of APNet generally tends to decrease across various values of $n$.
However, the decreasing tendency is not monotonic with small value of $n$ ($n=100$ and $n=1000$).
When $n=100$ or $1000$, the accuracy of APNet tends to decrease at first and then increase with distance ranging from 0.17 to 0.22.
As the value of $n$ increases (from the left sub-figure to the right one), the decreasing tendency of performance gradually stabilizes, presenting a linear relationship between the few-shot performance and calculated distance.
We argue this is because when a small number of training tasks is sampled (for example, when $n=100$ or $1000$), the sampled tasks can not cover the characteristics of the entire training data. 
Taking CUB dataset as an illustration, CUB dataset consits of 100 training categories.
In the 5-way 1-shot setting, each training task is composed of 5 categories sampled from a pool of 100 training categories.
During the training process, the number of possible sampled training tasks is a combinatorial number, specifically $C_{100}^5=75,287,520$, which is much larger than 100 and 1000.
Our experimental results also indicate that, despite the vast number of possible training tasks, stable decreasing tendency of few-shot performance can be achieved by sampling only $10,000$ or $100,000$ training tasks.

\textbf{Deeper Backbone.}
As mentioned previous sections, we have proven that TAD can serve as a metric to measure the adaptation difficulty on novel tasks for different FSL methods.
Here we consider how a deeper backbone affects this conclusion.
Following \cite{chen2019baseline++}, we use ResNet18 as backbones and train the five FSL models on CUB and SUN datasets.
Fig. \ref{fig:deeper backbone} shows the task distance and the corresponding accuracy of those models on 2,400 novel tasks.
As shown in Fig. \ref{fig:deeper backbone}, we observe similar phenomenon that with the increase of task distance, the accuracy of these models tends to decrease.
This indicates that the proposed TAD metric still works for different FSL methods with a deeper backbone model.

\input{overleaf/sections/tab_fig/ablation_deeper_backbone.tex}

\textbf{Varying number of categories.}
We next investigate the influence of number of categories in novel tasks.
In this exploration, we maintain a constant number of categories in training tasks while varying the number of categories in novel tasks, which involves a discrepancy in the number of categories between the training and novel tasks.
More specifically, we train various FSL models with 5-way 1-shot setting while evaluate them with 10-way/20-way 1-shot setting.
%In this scenario, the number of categories in training and novel tasks are not the same.
Fig. \ref{fig:varying ways} shows the distance and accuracy curves on CUB and SUN datasets with varying number of categories.
From Fig. \ref{fig:varying ways}, we have two observations: 
(1) TAD metric can still quantify the task relatedness and reflect adaptation difficulty on novel tasks with the discrepancy between training and novel tasks.
Fig. \ref{fig:varying ways} shows a similar phenomenon that with the increase of task distance, the accuracy of different FSL models tends to decrease.
(2) However, TAD metric becomes less applicable to some FSL models as the degree of discrepancy deepens.
For example, when novel tasks contain 20 categories, we observe that the accuracy of Baseline++ model experiences only marginal decline  (around 1\%) with increasing distance.

\input{overleaf/sections/tab_fig/ablation_varying_ways}

\begin{comment}

\paragraph{Predefined Attributes}
As our theory and proposed TAD metric rely on predefined attributes, the attribute set plays an important role in the process of measuring adaptation difficulty.
We next investigate the selection of attributes that are critical in the TAD metric.
    
\end{comment}

\subsection{\textcolor{black}{Comparison with Other Metrics}}
Here we present comparisons between proposed TAD and other metrics to show the effectiveness of it.
For comparing different metrics, we design a task selection experiment. 
More specifically, we select top 5\% novel tasks with the highest distances computed by different metrics, and then evaluate the accuracy of FSL models on these chosen tasks. 
The central hypothesis behind this experiment is that if a distance metric can better reflect task difficulty, then novel tasks with the highest distances should be more challenging.

\textbf{Comparative Methods.}
We compare our TAD metric with two distribution divergence metrics, which have been proposed in the few-shot learning or related area: 
(1) Frechet Inception Distance (\textbf{FID}) \cite{milbich2021ooDML}, FID is a metric to measure the distance between two image distributions by comparing their mean and covariance of representations. 
(2) Earth Mover’s Distance (\textbf{EMD}) \cite{oh2022domain-similarity}, EMD is a measure of dissimilarity between two distributions by considering the distance as the cost of moving image representations from one distribution to the other. 
The two above methods assume that the representation function learned from training categories can be directly applied to novel categories.
%Furthermore, we also compare our TAD metric with \textbf{Task2vec} \cite{achille2019task2vec}, which represents each task as an embedding, and the norm of embedding reflects task difficulty. 
%Note that Task2vec utilize the Fisher Information Matrix to quantify the task relatedness without assuming a common representation function.
%Following \cite{oh2022domain-similarity}, we use ResNet-101 pre-trained on ImageNet as the probe network to encode images for Task2Vec.

\textbf{Results.}
We compare these aforementioned methods with both original TAD (defined in Eq. (\ref{eq:origin})) and approximate TAD (defined in Eq. (\ref{eq:approximation})) on CUB and the cross-dataset scenario.
Tab. \ref{tab:comparison metrics cub} and \ref{tab:comparison metrics cross} illustrates the results of different methods. 
First of all, We can find that, with both human-annotated and auto-annotated attributes, original TAD (TAD-Orig) and approximate TAD (TAD-Approx) metrics significantly outperform other three methods in identifying more challenging novel tasks across all FSL models, demonstrating the effectiveness of TAD metrics. 
Secondly, TAD metrics can be applied to all FSL methods, while the FID and EMD metrics does not support MAML.
This is because MAML updates the feature extractor during adaptation, thereby violating the assumption of a common representation function between training and novel categories.
Finally, Tab. \ref{tab:comparison metrics cub} and \ref{tab:comparison metrics cross} also show that approximate TAD metric achieves similar or even better performance than the original one, which showcase that approximating Eq. (\ref{eq:origin}) with Eq. (\ref{eq:approximation}) is still effective and useful in measuring the adaptation difficulty on novel tasks for various FSL models.

\input{overleaf/sections/tab_fig/comparison_metrics_cub}

\input{overleaf/sections/tab_fig/comparison_metrics_cross}

\subsection{\textcolor{black}{Time Complexity}}
We next analyze the time complexity of original and approximate TAD metrics.
Computing the original TAD distance in Eq. (\ref{eq:origin}) requires finding the minimum weight perfect matching $M$ in a bipartite graph $G$, which is a combinatorial optimization problem.
The Hungarian algorithm \cite{kuhn1955hungarian} is commonly used to solve the matching problem, which employs a modified shortest path search in the augmenting path algorithm.
The running time of the Hungarian algorithm is $O(V^2\log V+VE)$, where $V$ is the number of vertices and $E$ is the number of edges in the bipartite graph $G$.
Assume that each training and novel task contain $C$ categories, thus the time complexity of original TAD is $O(C^3)$.
By simplifying the comparison of attribute conditional distribution between two tasks, the approximate TAD can avoid the need to seek the minimum weight perfect matching $M$ and achieve a constant time complexity of $O(1)$.
In Tab. \ref{tab:time complexity}, we compare the computation time of original and approximate TAD metrics on 2,400 novel tasks.
As we can see, the computational efficiency of approximate TAD greatly surpasses the original one, requiring only 0.7 seconds to compute across 2400 novel tasks, underscoring its advantage of ease of computation.
Furthermore, as shown in Tab. \ref{tab:time complexity}, the increase of number of ways (number of categories) in each novel task has significant influence on the computation time of the original TAD, while has negligible influence on the approximate TAD.
This observation validates that the time complexity of approximate TAD is independent of the number of categories in novel tasks.
Finally, the number of shots (number of labeled samples) has negligible influence on the computation time of the two metrics.
This is because both original and approximate TAD metrics rely solely on the attribute conditional distributions in training and novel tasks, making them independent of models and the number of labeled samples in novel tasks.


\input{overleaf/sections/tab_fig/time-complexity}

==> overleaf/sections/tab_fig/application_intervention.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.3\textwidth]{overleaf/plot/figures/experiments/test-time_cross.pdf}
    \caption{1-shot results of test-time intervention (\emph{mini}ImageNet$\rightarrow$CUB). We only show the accuracy of the intervened tasks.}
    \label{fig:test-time intervention}
\end{figure}

==> overleaf/sections/tab_fig/comparison_metrics.tex <==
\begin{table*}[]
\centering
\begin{tabular}{lllllllll}
\toprule
\multicolumn{1}{c}{Scenario} & \multicolumn{1}{c}{Metrics} & \multicolumn{1}{c}{MatchingNet} & \multicolumn{1}{c}{ProtoNet} & \multicolumn{1}{c}{RelationNet} & \multicolumn{1}{c}{Baseline++} & \multicolumn{1}{c}{APNet} & \multicolumn{1}{c}{MAML} & \multicolumn{1}{c}{mean} \\ \midrule
\multirow{5}{*}{CUB}           & FID                         & -2.34 (0.69)                    & -1.18 (0.93)                 & -1.58 (0.93)                    & -2.30 (0.91)                   & -1.72 (1.09)              & -                        & -                        \\
                             & EMD                         & -0.07 (1.33)                    & 0.48 (0.92)                  & 1.10 (0.77)                     & 0.67 (1.14)                    & 0.12 (0.96)               & -                        & -                        \\
                             & Task2Vec                    & -1.77 (2.57)                    & -0.14 (2.05)                 & -0.37 (1.76)                    & -                              & 0.79 (2.34)               & -                        & -                        \\ \cmidrule{2-9}
                             & TAD-Orig                    & -6.14 (1.23)                    & -6.67 (0.84)                 & -7.19 (0.79)                    & -4.49 (0.53)                   & -4.63 (1.05)              & -                        & -                        \\
                             & TAD-Average                 & \textbf{-8.03 (1.02)}                    & \textbf{-6.87 (0.76)}                 & \textbf{-8.22 (0.95) }                   & \textbf{-5.16 (1.02)}                   & \textbf{-6.96 (0.57) }             & -                        & -                        \\ \midrule
\multirow{5}{*}{miniImageNet$\rightarrow$ CUB}           & FID                         & -0.09 (0.41) & 0.01 (0.92) & -0.81 (0.85) & -0.49 (0.75) & -                         & -                        & -                        \\
                             & EMD                         & 1.73 (0.43) & 0.59 (0.93) & 0.86 (0.93) & 0.44 (0.69) & -                         & -                        & -                        \\
                             & Task2Vec                    & -0.45 (1.80)                               & -0.28 (1.18)                            & -0.10 (1.16)                               & -                              & -                         & -                        & -                        \\ \cmidrule{2-9}
                             & TAD-Orig                    & -3.01 (0.96)                               & -1.68 (0.60)                            & -4.25 (1.09)                               & -                              & -                         & -                        & -                        \\
                             & TAD-Average                 & -2.93 (0.78) & -2.22 (0.58) & -3.95 (0.90) & -2.94 (0.96) & -                         & -                        & -                        \\ \bottomrule
\end{tabular}
\caption{Comparison with different metrics in the task selection experiments. We run the experiments on CUB and cross-dataset (miniImageNet$\rightarrow$ CUB) situation. For the former, the human-annotated attributes are available, for the latter, the human-annotated attributes are unavailable, and we use auto-annotated attributes instead.  In all experiments, we run 10
times with different random seed then report the average results with standard deviation. The best results are in bold.}
\label{tab:comparison metrics}
\end{table*}

==> overleaf/sections/tab_fig/worst-case-intervention.tex <==
\begin{table*}[]
\centering
\begin{tabular}{ll|lllllllll}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{Sample Strategy}} & \multicolumn{1}{c|}{\multirow{2}{*}{Task Strategy}} & \multicolumn{3}{c}{ACC$_{20}$}                                                              & \multicolumn{3}{c}{ACC$_{60}$}                                                              & \multicolumn{3}{c}{ACC$_{120}$}                                                       \\
\multicolumn{1}{c}{}                                 & \multicolumn{1}{c|}{}                               & \multicolumn{1}{c}{5\%} & \multicolumn{1}{c}{10\%} & \multicolumn{1}{c|}{20\%}       & \multicolumn{1}{c}{5\%} & \multicolumn{1}{c}{10\%} & \multicolumn{1}{c|}{20\%}       & \multicolumn{1}{c}{5\%} & \multicolumn{1}{c}{10\%} & \multicolumn{1}{c}{20\%} \\ \midrule
\multirow{2}{*}{\textbf{Random}}                              & Random                                              & 50.9 (1.3)              & 51.9 (0.9)                        & \multicolumn{1}{l|}{51.7 (1.1)} & 55.1 (0.7)              & 55.9 (0.6)                        & \multicolumn{1}{l|}{55.7 (0.6)} & 57.9 (0.4)              & 58.5 (0.5)                        & 58.5 (0.5)                \\
                                                     & TAD                                                 & 52.8 (0.9)              & 52.4 (0.8)                        & \multicolumn{1}{l|}{53.5 (1.1)} & 56.3 (0.4)              & 56.2 (0.6)                        & \multicolumn{1}{l|}{56.8 (0.8)} & 58.8 (0.2)              & 58.8 (0.5)                        & 59.3 (0.6)                \\ \midrule
\multirow{2}{*}{\textbf{K-means}}                             & Random                                              & 51.5 (0.6)              & 51.7 (0.6)                        & \multicolumn{1}{l|}{51.4 (0.8)} & 55.4 (0.4)              & 55.6 (0.5)                        & \multicolumn{1}{l|}{55.6 (0.5)} & 58.1 (0.4)              & 58.3 (0.5)                        & 58.5 (0.4)                \\
                                                     & TAD                                                 & 52.8 (1.0)              & 52.8 (0.9)                        & \multicolumn{1}{l|}{53.5 (1.1)} & 56.4 (0.5)              & 56.5 (0.4)                        & \multicolumn{1}{l|}{57.3 (0.9)} & 58.9 (0.5)              & 59.2 (0.3)                        & 59.8 (0.7)                \\ \midrule
\multirow{2}{*}{\textbf{FDS}}                                 & Random                                              & -                       & -                        & \multicolumn{1}{l|}{-}          & -                       & -                        & \multicolumn{1}{l|}{-}          & -                       & -                        & -                         \\
                                                     & TAD                                                 & -                       & -                        & \multicolumn{1}{l|}{-}          & -                       & -                        & \multicolumn{1}{l|}{-}          & -                       & -                        & -                         \\ \bottomrule
\end{tabular}
\caption{Worst Case Intervention on CUB dataset.}
\label{tab:worst case intervention}
\end{table*}

==> overleaf/sections/theory.tex <==
\section{Theoretical Analysis on Generalization}
We have defined TAD metric to quantify the relatedness between tasks, further question is how the task relatedness affects the adaptation difficulty on novel tasks for different FSL models?
We try to explore this question in this section through theoretical analysis on generalization.
We first introduce a meta-learning framework with attribute learning to facilitate our theoretical analysis.
Then, we provide theoretical proof that establishes a connection between the proposed TAD metric and the generalization error bound on a novel task.

\subsection{A Specific Few-Shot Learning Framework}
\label{Sec 4.2.1}
To facilitate the subsequent theoretical analysis, we consider a meta-learning framework with attribute learning.
In this framework, a meta-learner $f_\theta: \mathcal{X}\rightarrow \mathcal{A}$ parameterized by $\theta$ learns the mapping from a sample $x\in\mathcal{X}$ to attributes $a\in\mathcal{A}$, and a task-specific base-learner $g_{\phi_i}: \mathcal{A}\rightarrow \mathcal{Y}_i$ parameterized by $\phi_i$ learns the mapping from attributes $a\in\mathcal{A}$ to a class label $y\in\mathcal{Y}_i$ for training task $\tau_i$.
During training, $f_\theta$ is meta-learned from $n$ different training tasks.
To adapt to a novel task $\tau_{j}'$, we fix $f_\theta$ and train a new base-learner $g_{\phi_{j}'}$ parameterized by $\phi_{j}'$ using few labeled samples $S_j'$. 

In the following theoretical deduction, we will denote $p_\theta(a,y)\triangleq p(f_{\theta}(x),y)$ as a joint distribution over $\mathcal{A}\times\mathcal{Y}$ induced by the meta-learned mapping $f_\theta$. 
Further, with the induced conditional distribution $p_\theta(a|y)$, we can compute the distance between task $\tau_i$ and $\tau_j'$ as 
\begin{align}
    d_\theta(\tau_i, \tau_{j}') &= \frac{1}{L\left|M\right|}\sum_{e_{kt}\in M} \sum_{l=1}^L d_{TV}(p_\theta^i(a^l|y_k), p_\theta^j(a^l|y_t)).
\end{align}
Note that $d(\tau_i, \tau_j')$ (as defined in Eq. (\ref{eq:dis_task})) computed based on $p(a|y)$ is the model-agnostic distance metric, while $d_\theta(\tau_i, \tau_j')$ is a model-related one since it relies on the meta-learned mapping $f_\theta$.

\subsection{Measuring Task Adaptation Difficulty via Attributes}
As for the above meta-learning framework, we provide theoretical analysis of the generalization error on a novel task, in terms of the proposed TAD metric.
We define the generalization error and empirical error of the meta-learner $f_\theta$ on novel task $\tau_{j}'$ as
\begin{align*}
    \epsilon(f_\theta, \tau_{j}')&=\mathbb{E}_{(x,y)\sim \mathcal{D}_{j}'}[\mathbb{I}(g_{\phi_{j}'}(f_\theta(x))\neq y)], \\
    \hat{\epsilon}(f_\theta, \tau_{j}')&=\frac{1}{m_{j}'} \sum_{k=1}^{m_{j}'}\mathbb{I}(g_{\phi_{j}'}(f_\theta(x_k))\neq y_k), \notag
\end{align*}
where $\phi_{j}'$ is the parameters of $g_\phi$ learned from labeled samples $S_{j}'$ given $f_\theta$, and ${m_j'}=\left|S_{j}'\right|$ is the number of labeled samples in $S_{j}'$.
$\mathbb{I}$ denotes the indicator function.
Similarly, we can define the generalization error $\epsilon(f_\theta, \tau_i)$ and empirical error $\hat{\epsilon}(f_\theta, \tau_i)$ for training task $\tau_i$.
With these definitions, we will proceed by introducing an auxiliary lemma, and then stating our main theoretical results.
All detailed proofs of the following lemma and theorems are in the Appendix A. 

\begin{lemma}
    Let $\mathcal{A}$ be the attribute space, $L$ be the number of attributes.
    %For the conditional distribution $p(a|y)$, 
    Assume all attributes are independent of each other given the class label, i.e. $p(a|y) = \prod_{l=1}^Lp(a^l|y)$.
    For all $a_i \in \mathcal{A}$ and any two categories $y_k, y_t$, the following inequality holds:
    \begin{equation}
        \sum_{a_i\in\mathcal{A}}\left|p(a_i|y_k)-p(a_i|y_t)\right| \leq d_{\mathcal{A}}(y_k, y_t) +  \Delta,
        \label{eq:distance ineq}
    \end{equation}
    where $d_{\mathcal{A}}(y_k, y_t)$ is the distance as defined in Eq.(\ref{eq:dis_category}) and $\Delta=\sum_{a_i\in\mathcal{A}}\frac{1}{2L}\sum_{l=1}^L(p(a^l_i|y_k)+p(a^l_i|y_t))$.
    \label{lemma 1}
\end{lemma}
Lemma \ref{lemma 1} says that under the attribute conditional independence assumption, the distance between two attribute conditional distributions $p(a|y_k), p(a|y_t)$ over attribute space $\mathcal{A}$ is %be spanned by 
bounded by the defined distance $d_{\mathcal{A}}(y_k, y_t)$ and a non-negative term $\Delta$.
This result enables us to make use of the defined TAD metric in deriving the generalization error bound, leading to the following theoretical results.

\begin{theorem}
    With the same notation and assumptions as in Lemma \ref{lemma 1}, %let $\mathcal{H}$ be the hypothesis space of the meta-learning method (introduced in Sec. 4.2) with VC-dimension $d$, 
    let $\mathcal{H}$ be the hypothesis space with VC-dimension $d$, 
    $f_\theta$ and $g_\phi$ be the meta-learner and the base-learner as introduced in Sec \ref{Sec 4.2.1} respectively. 
    Denote $g_{\phi^*}$ as the best base-learner on some specific tasks given a fixed meta-learner $f_\theta$.
    For any single training task $\tau_i=(\mathcal{D}_i, S_i)$ and a novel task $\tau_{j}'=(\mathcal{D}_{j}', S_{j}')$, suppose the number of categories in the two tasks is the same, then with probability at least $1-\delta$, $\forall g_\phi\circ f_\theta\in\mathcal{H}$, we have 
    \begin{align}
         \epsilon(f_\theta, \tau_{j}')&\leq 
            \hat{\epsilon}(f_\theta, \tau_i) + \sqrt{\frac{4}{m_i}(d\log\frac{2em_i}{d}+\log\frac{4}{\delta})}
            \notag \\ &+ d_\theta(\tau_i, \tau_{j}') + \Delta' + \lambda, 
            \label{theorem 1}
    \end{align}
    where $\lambda=\lambda_i+\lambda_j'$ is the generalization error of $g_{\phi^*}$ and $f_\theta$ on the two tasks, i.e., 
    % and $\lambda_i, \lambda_t$ are the generalization error of the best base-learner $g_{\phi^*}$ with a fixed $f_\theta$ on task $\tau_i, \tau_t'$ respectively.
    $\lambda_i=\mathbb{E}_{(x,y)\sim \mathcal{D}_i}[\mathbb{I}(g_{\phi_{i}^*}(f_\theta(x))\neq y)]$, $\lambda_j'=\mathbb{E}_{(x,y)\sim \mathcal{D}_{j}'}[\mathbb{I}(g_{\phi_{j}'^*}(f_\theta(x))\neq y)]$. $\Delta'$ is a term depending on learned base-learners $g_{\phi_i}, g_{\phi_j'}$ and the best base-learners $g_{\phi_i^*}, g_{\phi_j'^*}$.
    \label{theorem 1}
\end{theorem}

Theoretically, the generalization error on a novel task is bounded by the the training task empirical error $\hat{\epsilon}(f_\theta, \tau_i)$ plus four terms: 
the second term $d_\theta(\tau_i, \tau_{j}')$ is the model-related distance between $\tau_i$ and $\tau_{j}'$, which is derived based on Lemma \ref{lemma 1};
the third term $\Delta'$ reflects the classification ability of $g_\phi$, which converges to zero if the learned base-learners are equal to the best ones for both tasks;
the last term $\lambda$ is the generalization error of $f_\theta$ and $g_{\phi^*}$, which depends on the attribute discrimination ability of $f_\theta$ and the hypothesis space of base-learner $g_\phi$.
% For a complex neural networks, if $f_\theta$ has a good attribute discrimination ability, this term usually converges to zero.
For a reasonable hypothesis space, if $f_\theta$ has a good attribute discrimination ability on both tasks, the last term usually converges to zero. 
Next we generalize this bound to the setting of $n$ training tasks.

\begin{corollary}
   With the same notation and assumptions as Theorem 1, 
    for $n$ training tasks $\{\tau_i\}_{i=1}^n$ and a novel task $\tau_{j}'$, 
    define $\hat{\epsilon}(f_\theta, \tau_{i=1}^n)=\frac{1}{n}\sum_{i=1}^n \hat{\epsilon}(f_\theta, \tau_i)$, then with probability at least $1-\delta$, $\forall g_\phi\circ f_\theta\in\mathcal{H}$, we have
    \begin{align}
        \epsilon(f_\theta, \tau_{j}')&\leq 
            \hat{\epsilon}(f_\theta, \tau_{i=1}^n) + \frac{1}{n}\sum_{i=1}^n\sqrt{\frac{4}{m_i}(d\log\frac{2em_i}{d}+\log\frac{4}{\delta})}
            \notag \\ 
            & + \frac{1}{n}\sum_{i=1}^n d_\theta(\tau_i, \tau_{j}') + \Delta' + \lambda, 
            \label{eq:corollary 1}
    \end{align}
    where $\lambda=\frac{1}{n}\sum_{i=1}^n \lambda_i + \lambda_j'$, and $\Delta'$ is a term depending on the learned base-learners $\{g_{\phi_i}\}_{i=1}^n, g_{\phi_j'
    }$ and the best base-learners $\{g_{\phi_i^*}\}_{i=1}^n, g_{\phi_j'^*}$.
    \label{corollary 1}
\end{corollary}
Corollary \ref{corollary 1} is a straightforward extension of Theorem \ref{theorem 1}, in which we consider multiple training tasks instead of a single training task.
In Corollary \ref{corollary 1}, the generalization error on a novel task $\tau_{j}'$ is  bounded partially by the average distance between task $\tau_{j}'$ and $n$  training tasks.
Note that the distance $d_\theta(\tau_i, \tau_j')$ used in the bound is %in the bound is defined on the mapping $f_\theta$, which maps each sample point $x\in\mathcal{X}$ to $a\in\mathcal{A}$, thus is a 
model-related.
Next, we further derive the relationship between model-related distance and model-agnostic distance as follows.

\begin{definition}[\textcolor{black}{$\epsilon$-approximation mapping}]
    \label{definition 1}
    A meta-learner $f_{\theta}:\mathcal{X}\rightarrow\mathcal{A}$, parameterized by $\theta$, is termed an $\epsilon$-approximation mapping for $n$ training tasks $\{\tau_i\}_{i=1}^n$ if $\|f_\theta-f\|<\epsilon$,
    where $f:\mathcal{X}\rightarrow\mathcal{A}$ is the true labeling mapping for $n$ training tasks.
\end{definition}

\begin{theorem}
   \label{theorem 2}
    With the same notation and assumptions as in Corollary \ref{corollary 1}, assume that the conditional distribution $p(x|a^l)$ is task agnostic, 
    \textcolor{black}{and the meta-learner $f_{\theta}$ is an $\epsilon$-approximation mapping for $n$ training tasks.
    If $\epsilon$ tends to zeros, the following equality holds:}
    \begin{align}
            \frac{1}{n}\sum_{i=1}^nd_\theta(\tau_i, \tau_{j}')&\leq\frac{1}{n}\sum_{i=1}^nd(\tau_i, \tau_{j}').
    \end{align}
\end{theorem}

Theorem \ref{theorem 2} shows that when  the meta-learner $f_{\theta}$ is in the proximity of the true labeling function $f:\mathcal{X}\rightarrow\mathcal{A}$ for $n$ training tasks, the model-related average distance $\frac{1}{n}\sum_{i=1}^nd_\theta(\tau_i, \tau_{j}')$ can be bounded by the average TAD $\frac{1}{n}\sum_{i=1}^nd(\tau_i, \tau_{j}')$.
%Based on the universal approximation theorem  \cite{hornik1989universe, farago1993strong} and the same assumption as in Theorem \ref{theorem 2}, if $g_\phi\circ f_\theta$ is a complex enough neural network, the second and fourth terms on the r.h.s. of Eq.~(\ref{eq:corollary 1}) in Corollary \ref{corollary 1} will converge to $0$, the first term $\hat{\epsilon}(f_\theta, \tau_{i=1}^n)$ and $\frac{1}{n}\sum_{i=1}^n \lambda_i$ in the last term will converge to Bayes risk \cite{dougherty2012prc}.
With the same assumption as in Theorem \ref{theorem 2}, the fourth terms on the r.h.s. of Eq.~(\ref{eq:corollary 1}) in Corollary \ref{corollary 1} will converge to $0$.
Based on the universal approximation theorem  \cite{hornik1989universe, farago1993strong}, if $g_\phi\circ f_\theta$ is a complex enough neural network, the first term $\hat{\epsilon}(f_\theta, \tau_{i=1}^n)$ and $\frac{1}{n}\sum_{i=1}^n \lambda_i$ in the last term will converge to Bayes risk \cite{dougherty2012prc}.
We assume the Bayes risk is small enough, so that it can be ignored.
In this case, the generalization error on novel task $\tau_j'$ is only bounded by a complexity term,  $\lambda_j'$ and the average TAD, i.e. $\epsilon(f_\theta,\tau_j')\leq \frac{1}{n}\sum_{i=1}^n\sqrt{\frac{4}{m_i}(d\log\frac{2em_i}{d}+\log\frac{4}{\delta})} + \lambda_j'+\frac{1}{n}\sum_{i=1}^nd(\tau_i, \tau_j')$.
Note that the average TAD is independent of models, thus we can rely solely on the TAD to measure the adaptation difficulty of each novel task, without the need for training any models.

Note that the meta-learner $f_\theta$ discussed in the theoretical derivation maps images to the attribute space, whereas in various popular FSL methods, $f_\theta$ (such as metric-based and transfer-based methods) maps images  into a generic representation space.
Thus, the attribute-based meta-learning framework can be consider a special form of various FSL methods.
We will empirically verify that the TAD metric is applicable to attribute-based meta-learning method and other FSL methods, even if some of them do not learn attributes explicitly.
